A Survey of Neural Code Intelligence: Paradigms, Advances and Beyond

Neural Code Intelligence -- leveraging deep learning to understand, generate, and optimize code -- holds immense potential for transformative impacts on the whole society. Bridging the gap between Natural Language and Programming Language, this domain has drawn significant attention from researchers in both research communities over the past few years. This survey presents a systematic and chronological review of the advancements in code intelligence, encompassing over 50 representative models and their variants, more than 20 categories of tasks, and an extensive coverage of over 680 related works. We follow the historical progression to trace the paradigm shifts across different research phases (e.g., from modeling code with recurrent neural networks to the era of Large Language Models). Concurrently, we highlight the major technical transitions in models, tasks, and evaluations spanning through different stages. For applications, we also observe a co-evolving shift. It spans from initial endeavors to tackling specific scenarios, through exploring a diverse array of tasks during its rapid expansion, to currently focusing on tackling increasingly complex and varied real-world challenges. Building on our examination of the developmental trajectories, we further investigate the emerging synergies between code intelligence and broader machine intelligence, uncovering new cross-domain opportunities and illustrating the substantial influence of code intelligence across various domains. Finally, we delve into both the opportunities and challenges associated with this field, alongside elucidating our insights on the most promising research directions. An ongoing, dynamically updated project and resources associated with this survey have been released at https://github.com/QiushiSun/Awesome-Code-Intelligence.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> sqs_custom.tex <==

% \definecolor{pjlabblue}{RGB}{65,126,155}
% \definecolor{lightbluegray}{RGB}{240,245,250}
% \definecolor{icyrockblue}{RGB}{240,245,255}

% % #417E9B
% % \definecolor{}{}{}

% %%%
% \usepackage{tcolorbox}
% \newtcolorbox{finding}{
% colframe=black!80,
% colback=icyrockblue,
% fonttitle=\bfseries,
% coltitle=black,
% left=3pt,
% right=3pt,
% top=3pt,
% bottom=3pt,
% boxrule=0.4mm,
% arc=3mm
% }
% %%%

==> tables/nl2code-eval.tex <==
% \begin{table}[ht]
%   \centering
%   % \footnotesize
%   \begin{tabular}{lcc|c|c}
%     \toprule
%     \textbf{Model} & \textbf{Ver.} & \textbf{Size} & \textbf{HumanEval} & \textbf{MultiPL-E} \\
%     \midrule
%     CodeX-001 & - & - & 33.5 & 26.1 \\    
%     \midrule
%     CodeGeeX2 & - & 6B & 36.0 & 24.5 \\
%     \midrule
%     \multirow{4}{*}{CodeLlaMA} & \multirow{3}{*}{Base} & 7B & 31.7 & 29.2 \\
%                                &                       & 13B & 36.0 & 35.4 \\
%                                &                       & 34B & 48.2 & 41.0 \\
%     \cmidrule(lr){2-5}
%                                & Instruct & 34B & 41.5 & 36.1 \\
%     \midrule
%     \multirow{3}{*}{DeepSeek-Coder} & Base & 1B & 34.8 & 28.3 \\
%     \cmidrule(lr){2-5}
%                                     & \multirow{2}{*}{Instruct} & 7B & 78.6 & 66.1 \\
%                                     &                           & 33B & 79.3 & 69.2 \\
%     \midrule
%     \multirow{2}{*}{StarCoder} & - & 15.5B & 33.6 & 25.3 \\
%                                & Plus & 15.5B & 26.2 & 21.4 \\
%     \midrule
%     \multirow{2}{*}{Lemur} & Base & 70B & 35.4 & 30.4 \\
%                            & Chat & 70B & 61.0 & 42.9 \\
%     \midrule
%     WizardCoder & - & 15B & 57.3 & 30.8 \\
%     \midrule
%     LlaMA2 & Chat & 70B & 31.1 & 22.6 \\
%     \midrule
%     GPT-3.5-Turbo & - & - & 76.2 & 64.9 \\
%     \midrule
%     GPT-4 & - & - & 84.1 & 76.5 \\
%     \bottomrule
%   \end{tabular}
%   \caption{Model Performance Comparison \pak}
%   \label{tab:nl2code-eval}
% \end{table}

% \begin{figure*}[t]
%    \begin{center}
%    {\includegraphics[width=\linewidth]{figures/opensource-eval.pdf}} 
%    \end{center}
% \caption{The Pass@1 performance of open-source CodeLLMs on HumanEval, showing the result for each model across different sizes and versions.}
% \label{fig:nl2code-eval}
% \end{figure*}


==> tables/text2sql.tex <==
\begin{table}[ht]
    \centering
    \footnotesize
    \caption{\emph{\# Schema} refers to the number of tables covered in the datasets. \sqs{@ xfz, consider moving this into text?}}
    \begin{tabular}{l|c|c|c}
        \toprule
        \textbf{Datasets} & \textbf{Size} & \textbf{\# Schema} & \textbf{Sources} \\
        \midrule
        ATIS~\citep{dahl1994expand} &11,653 & 27 &flights etc. \\
        Spider~\citep{yu2018spider} &10,181 &1,020 & 138 domains \\
        Sparc~\citep{yu2019sparc} &12,726 &1,020 & 138 domains \\
        Cosql~\citep{yu2019cosql} & 15,598 &1,020 & dialogues, 138 domains \\
        WikiSQL~\citep{zhong2017seq2sql} &80,654 &24,241 &Wikipedia \\
        WikiTQ~\citep{panupong2015comp} &22,033 &2,108 &Wikipedia  \\
        Squall &11,276 &2,108 & Wikipedia \\
        KaggleDBQA & 272 & 18 & Web Database\\
        \bottomrule
    \end{tabular}
    \label{tab:text2sql_benchmark}
\end{table}


% Spider~\citep{yu2018spider}
% Sparc~\citep{yu2019sparc}
% Cosql~\citep{yu2019cosql}
